Power Grid Simulation using Matrix Exponential Method with Rational Krylov Subspaces

One well adopted power grid simulation methodology is to factorize matrix once and perform only backward forward substitution with a deliberately chosen step size along the simulation. Since the required simulation time is usually long for the power grid design, the costly factorization is amortized. However, such fixed step size cannot exploit larger step size for the low frequency response in the power grid to speedup the simulation. In this work, we utilize the matrix exponential method with the rational Krylov subspace approximation to enable adaptive step size in the power grid simulation. The kernel operation in our method only demands one factorization and backward forward substitutions. Moreover, the rational Krylov subspace approximation can relax the stiffness constraint of the previous works. The cheap computation of adaptivity in our method could exploit the long low frequency response in a power grid and significantly accelerate the simulation. The experimental results show that our method achieves up to 18X speedup over the trapezoidal method with fixed step size.

==> sub-krylov_approx.tex <==
The computation of the matrix exponential 
\begin{eqnarray}
\label{eq:exp_taylor}
e^{\mbf A}\mbf v:=  \mbf {(I + A + \frac{A^2}{2!} + ... +\frac{ A^{n-1}}{k!}+...)v}. 
\end{eqnarray}
is extremely expensive.  
Thanks to well-known Krylov subspace algorithm~\cite{weng2012time, weng2012circuit, Hochbruck97, Saad92}. 

The Krylov subspace spans by the basis of $m$ vector
 \begin{eqnarray}
\label{eq:kryspan}
{\rm K_m}\left(\mbf{A}, \mbf{v}\right) := span\{\mbf {v, Av, A^2v, ..., A^{n-1}v}\}. 
\end{eqnarray}
Generally, the orthogonal bases of Krylov subspace can be constructed from Arnoldi or Lanczos process. 
 \begin{eqnarray}
\label{eq:kryspan}
\mbf {AV_m} =  \mbf {V_mH_m+H}(m+1,m)\mbf {v_{m+1}e^T_m}
\end{eqnarray}
where $\mbf{H_m}$ is Hessenberg matrix, $\mbf e_m$ is the $m$th unit vector with dimension $m \times 1$.
Assume $ \mbf {V^{T}_mAV_m =  H_m }$.
Therefore, $e^{\mbf{A}}\mbf{v}$ can be projected onto the Krylov 
subspace ${\rm K_m}\left(\mbf{A}, \mbf{v}\right)$ with dimension of $m$. 
Then~(\ref{eq:exp_taylor}) is evaluated by 
\begin{eqnarray}
\label{eq:Krylov_exp}
e^{\mbf A} \mbf v  \approx
 \mbf {V_m} \mbf {V^T_m}  e^{\mbf A} \mbf {V_m}  \mbf {V^T_m v}  = || \mbf v || \mbf {V_m} e^{\mbf H_m} \mbf e_1 
\end{eqnarray}
It is noted that in experiment for circuit simulation, the order $m$ is usually small, the overall computational complexity of exponential operator is greately reduce, so the scalability of MEXP is better than traditional implicit methods. 
The works in~\cite{weng2012time, weng2012circuit} use $\mbf{C}^{-1}(\mbf{G}\mbf{v})$ 
instead of computing $\mbf{C}^{-1}$ explicitly. 
These works claim solving $\mbf{C}$ is easier than $(\mbf{C}/h+\mbf{G})$ of implicit methods 
because $\mbf{C}$ has 
fewer non-zeros and better structure that can favor direct and iterative sparse solvers. 
However, if the circuit system is stiff or even singular $w.r.t.$ $\mbf C$, which will hamper the efficiency of calculation.
The Krylov subspace method, using matrix $\mbf A$ directly to form the bases, needs a large $m$ 
or a small $h$ to provide sufficient resolution 
to the spectrum of $\mbf{A}h$. Besides that, the large storage of $m$ bases for the high stiffness limits the size of circuit. 
We will address the issue in Section~\ref{sec:rational_krylov}. 
 

